Consider the Alternatives: Navigating Fairness-Accuracy Tradeoffs via Disqualification

In many machine learning settings there is an inherent tension between fairness and accuracy desiderata. How should one proceed in light of such trade-offs? In this work we introduce and study $\gamma$-disqualification, a new framework for reasoning about fairness-accuracy tradeoffs w.r.t a benchmark class $H$ in the context of supervised learning. Our requirement stipulates that a classifier should be disqualified if it is possible to improve its fairness by switching to another classifier from $H$ without paying "too much" in accuracy. The notion of "too much" is quantified via a parameter $\gamma$ that serves as a vehicle for specifying acceptable tradeoffs between accuracy and fairness, in a way that is independent from the specific metrics used to quantify fairness and accuracy in a given task. Towards this objective, we establish principled translations between units of accuracy and units of (un)fairness for different accuracy measures. We show $\gamma$-disqualification can be used to easily compare different learning strategies in terms of how they trade-off fairness and accuracy, and we give an efficient reduction from the problem of finding the optimal classifier that satisfies our requirement to the problem of approximating the Pareto frontier of $H$.

==> draft_bits.tex <==
\section{Learning optimal agnostic Pareto balanced classifiers}

\todo{
Sketch:
\begin{itemize}
    \item Learning from finite samples:
    
    \begin{itemize}
        \item Define $\hat{R}$, sample-version of disqualification relation
        
        \item define approximate disqualification and approximate agnostic Pareto fairness (addition of an additive slack $\alpha$, crucial for generalization)
        
        \item uniform convergence: given $m=g(\alpha, \delta, VC(\H))$ samples, w.p at least $1-\delta$ $\hat{R^\alpha} = R^\alpha$. i.e., $h'$ disqualifies $h$ on the sample iff it does so on $\P$.
    \end{itemize}
    
    \item The approximate fair-ERM problem: given $\H$, $\alpha$ and $\gamma$, find $h \in \Delta(\H)$ that minimizes loss subject to approximate agnostic fairness
    
    \item information theoretic learnability follows directly from the uniform convergence argument
    
    \item Remaining question: efficient optimization
    
    \begin{itemize}
        \item reduce approximate fair ERM to optimal disqualification
        
        \item informally, optimal disqualification is reduced to whether disqualification specifies a convex constraint
        
        \item For our setting, even for simplest $\H$, answer  is no
        
        \item ``convex relaxation'': switch imbalance to $\ell_2$ loss. (is this the first time I introduce it? if yes, need to show this relaxation makes sense because main axiom can be satisfied for $f=c$, and argue why a solution exists).
        
        \item hopefully we can prove: for every $\gamma$, can \emph{efficiently} solve for something that is $(\gamma, \alpha=g(\gamma), \H)$ fair when $\H$ is linear.
    \end{itemize}
    
    
\end{itemize}
}

We are interested in the problem of optimizing for accuracy, subject to a hard constraint on fairness (agnostic Pareto balance). We refer to this as the \emph{approximate fair-ERM} problem:


\begin{equation}
\label{prob:fair-erm}
    \min_{h \in \Delta(\H)} {\ell_A}(h) \quad \text{subject to} \quad h \,\, \text{satisfying} \,\, (\ell_A, \ell_B, \alpha, \gamma, \H)-\text{agnostic Pareto balance}
\end{equation}

The empirical version of this problem is

\begin{multline}
\label{prob:sample-fair-erm}
    \min_{h \in \Delta(\H)} \widehat{\ell_A}(h)  \quad \text{subject to} \,\, \forall h' \in \H, \\ \widehat{dLossImb}(h; \ell_B)-\widehat{dLossImb}(h'; \ell_B) \leq \alpha +  f_\gamma^{\ell_A, \ell_B} \br{\max \set{0, \,\, \widehat{\ell_A}(h')-\widehat{\ell_A}(h)}}
\end{multline}

Next, we define the \emph{optimal disqualification} problem: given a fixed classifier $p$ and a class $\H$, find the most accurate classifier that disqualifies $p$:

\begin{multline}
\label{problem:sample-opt-disq}
    \min_{h \in \Delta(\H)} \widehat{\ell_A}(h)  \quad \text{subject to}  \\ \widehat{dLossImb}(p; \ell_B)-\widehat{dLossImb}(h; \ell_B) > \alpha +  f_\gamma^{\ell_A, \ell_B} \br{\max \set{0, \,\, \widehat{\ell_A}(h)-\widehat{\ell_A}(p)}}
\end{multline}

\begin{lemma}
If we can efficiently solve (\ref{problem:sample-opt-disq}) then we can efficiently solve (\ref{prob:sample-fair-erm}).
\end{lemma}

So we turn to the optimal disqualification problem. First we need to do something with the max in the constraint -- we can simply convert it to two problems:the first will attempt to find a strictly more accurate disqualifiying classifier, whereas the second will attempt to find a less accurate disqualifying classifier:

\begin{multline}
\label{problem:sample-opt-disq1}
 \min_{h \in \Delta(\H)} \widehat{\ell_A}(h)  \quad \text{subject to} \quad  \widehat{\ell_A}(h)  < \widehat{\ell_A}(p) , \quad  \widehat{dLossImb}(h; \ell_B) < \widehat{dLossImb}(p; \ell_B) - \alpha 
\end{multline}

\begin{multline}
\label{problem:sample-opt-disq2}
 \min_{h \in \Delta(\H)} \widehat{\ell_A}(h)  \quad \text{subject to} \quad \widehat{\ell_A}(h)  \geq \widehat{\ell_A}(p) , \\ \widehat{dLossImb}(h; \ell_B) + f_\gamma^{\ell_A, \ell_B} \br{ \widehat{\ell_A}(h)-\widehat{\ell_A}(p)} < \widehat{dLossImb}(p; \ell_B) - \alpha 
\end{multline}

We will now assume that $\H=\H_w$ (linear classifiers), so $\Delta(\H) = \H$, and we are in the setting in which $\ell_A$ is the squared loss and $\ell_B$ is the expected zero one loss. \gal{Do we want to think about general classes? For general $\H$, it will still be true that everything is convex if I optimize over $\H$ itself. So it reduces to efficient agnostic learning with the squared loss (though I don't know  results for that).  The problem is with optimizing over $\Delta(\H)$ -- I would have wanted one parameter per $h \in \H$ (variables are the convex combination parameters), but then the squared loss is no longer convex in that representation.}

Note that the first problem , (\ref{problem:sample-opt-disq1}), is simply a convex problem: the objective and first constraint are convex because $\widehat{\ell_A}(h_w)$ is convex in $w$, and the second constraint is also convex because $\widehat{dLossImb}(h; \ell_B)$ is linear in $w$.

For the second problem, note that the first constraint is concave -- however, we can eliminate it, since we will only be solving (\ref{problem:sample-opt-disq2}) in the case that problem (\ref{problem:sample-opt-disq1}) did not return a solution, in which case this constraint is satisfied.

\begin{multline}
\label{problem:sample-opt-disq2-variant}
 \min_{h \in \Delta(\H)} \widehat{\ell_A}(h)  \quad \text{subject to} \quad  \widehat{dLossImb}(h; \ell_B) + f_\gamma^{\ell_A, \ell_B} \br{ \widehat{\ell_A}(h)-\widehat{\ell_A}(p)} < \widehat{dLossImb}(p; \ell_B) - \alpha 
\end{multline}

We are therefore left with the question of whether the function $\widehat{dLossImb}(h_w; \ell_B) + f_\gamma^{\ell_A, \ell_B} \br{ \widehat{\ell_A}(h_w)-\widehat{\ell_A}(p)} $ is convex in $w$. Unfortunately, in this case the answer is no: the argument for $f$ is convex in $w$, but $f(a)\propto \sqrt{a}$ is a concave function and the composition of a concave function with a convex function is not convex.

On the other hand, we can prove a positive result for the setting in which $\ell_A = \ell_B = \ell^2$. 

\begin{lemma}
When $\gamma \geq \mu \beta$ and $\ell_A = \ell_B = \ell^2$, problem (\ref{problem:sample-opt-disq2-variant}) can be solved efficiently.
\end{lemma}

\gal{I don't see why this is good enough. It only says I can solve the initial problem when $\gamma$ is not too small, but what about the cases in which it is too small? Intuitively, I can output $h_0$ (the optimal perfectly balanced classifier) and argue that since $\gamma$ is small, returning $h_0$ (as opposed to the actual optimum) can't be too bad. But I don't know in what sense this is true.}

Recall that in this setting, $f_\gamma^{\ell_A, \ell_B}(a) = c \cdot a$, w here $c = \frac{\gamma}{\mu \cdot \beta}$. 
So it's left to prove that 

\begin{equation*}
    g(w) = \widehat{dLossImb}(h_w; \ell^2) + c \cdot \widehat{\ell^2}(h_w) 
\end{equation*}

is convex in $w$.

Assume w.l.o.g that the imbalance of. $h$ is in favour of $T$; then, recall that the empirical loss imbalance is defined as
$\sum_{i: g_i = T, y_i = 1}\ell((h_w(x_i), y_i) - \sum_{i: g_i = S, y_i = 1}\ell((h_w(x_i), y_i)$. We can therefore re-write $g(w)$ as

\begin{equation*}
    g(w) = c\cdot \sum_{i:  y_i = 0}\ell((h_w(x_i), y_i) + (c+1) \cdot \sum_{i: g_i = T, y_i = 1}\ell((h_w(x_i), y_i) + (c-1) \cdot \sum_{i: g_i = S, y_i = 1}\ell((h_w(x_i), y_i)
\end{equation*}

Since by our assumption $c\geq 1$, $g(w)$ is convex (as a sum of convex functions).

\gal{Ugh, this isn't a very interesting result. 
}



%Do we even need / use $\gamma$ is any meaningful way, so far? Right now it's just there, not doing much except interpolation between accuracy alone / balance alone.

\section{Experiments}
 
 Auditing problem: given $h$ and $\H$, find the minimal $\gamma$ such that $h$ is $(\gamma, \H)$-agnostic-Pareto-balanced.
 
 Learning problem: given $\H$ and $\gamma$, find the most accurate $(\gamma, \H)$-fair classifier.

Empirically, for me the interesting question here is the auditing one for general class $\H$ (e.g. non-convex), and in particular, how fair is the ERM (or other particular strategies).

\gal{Is it true that anytime there is no loss mismatch (i.e. $\ell_A = \ell_B$, but they aren't necessarily $\ell^2$ - for example for Logistic Regression this might be logistic loss), the scaling should be linear?
I think it would be nice, because this could be the convex relaxation: pick any convex loss $\ell$ and use  $\ell_A = \ell_B = \ell$. We need to show that when $f$ is linear, the Bayes optimal is still 1-fair -- hopefully this is true.}


 Graphically, when $f_\gamma(a) = \gamma\cdot c\cdot a$, this looks as follows:


So $h_{ERM}$ is fair if the highlighted area is non-empty. We can use heuristics to try to find points in this area.  For example, we can add to the objective a penalty that corresponds to the loss imbalance (for various levels of $\lambda$), and plot what we receive. 

\gal{I think this is what I coded up in the past - would be good to come back to this and try to generate some nice graphs, for different groups on the Adult dataset!}



==> removed_bits.tex <==
\section{On the tension between fairness and accuracy}

An important motivation for our work is the inherent tension between fairness and accuracy \cite{}. For a definition such as Demographic parity, this is clear: even the ideal predictor (that predicts the true binary label $y$ of every $x$) is not fair when the base rates between the groups differ. This is alleviated by a definition like balance or Equal Opportunity -- but only when the learning procedure is unrestricted. It is not generally the case that the most accurate predictor in a bounded class $\H$ will be fair, even approximately. \footnote{See \cite{hebert2017calibration}'s ``rainy days'' example for a simple illustration. One way to think about balance is in the framework of metric fairness \cite{dwork2012fairness}: the positives of $T$ are similar to the positives of $S$ (in that both have the label $y=1$), and should therefore receive similar predictions. In practice, inherent uncertainty or missing features could mean that the positives of each group aren't really similar -- and that the maximally accurate and fair classifier is completely hypothetical.} A naive way to address this would be to opt, instead, for a sufficiently fair classifier - e.g. one whose imbalance is at most $\alpha$. But what is an appropriate level $\alpha$? We argue that classifiers could be imbalanced for very different reasons -- so a criterion that only considers the imbalance level is inherently limited. 



\begin{figure}[htbp!]
\centering
\captionsetup{width=0.9\linewidth}

\includegraphics[width=1.0\linewidth]{balance_problem.pdf}
\caption{In both figures, $h_w(x) = \sigma\langle w, x \rangle$ is imbalanced: the positive of $T$ receive an average score of $\approx 1$, while the positive of $S$ receive an average score of $\approx 1/2$. On the other hand, $h_{w_a}$ and $h_{w_b}$ are both perfectly balanced: under $w_a$ the positives of both groups receive an average prediction of $0.5$, while under $w_b$ both receive an average prediction of $1.0$.  }
\label{fig:balance-issue}
\end{figure}


For a simplified example, consider the two scenarios described in Figure
\ref{fig:balance-issue}. In this example, individuals from $T$ are denoted in blue, and individuals from $S$ are denoted in green. In both cases the data for $T$ is perfectly separable, and $h_w(x)$ predicts a value in $[0,1]$ according to the normalized distance from the hyper-plane denoted by $w$ (solid black line). Note that this classifier, tailored for $T$, is significantly imbalanced: in both cases the average prediction for $T^+$ is approximately $1.0$, whereas the  average prediction for $S^+$ is approximately $0.5$, so $Imb(h_w) = 0.5$. However, intuitively, the two scenarios are very different. In (b), this classifier is clearly unfair. For example, taking into account $S$ would result in the classifier $h_{w_b}$. Now the average prediction for $S^+$ is also approximately 1.0 and so this classifier is perfectly balanced. On the other hand, in (a), the data for $S$ is completely inseparable, so there is no genuine way to improve the predictions for $S^+$. For example, $h_{w_a}$ is one balanced predictor, but it achieves balance not by increasing the scores of $S^+$ but by decreasing the scores of $T^+$. In conclusion, while balance is an intuitively desirable property, on its own it does not allow us to make distinctions between seemingly very different scenarios, such as (a) and (b) in Figure \ref{fig:balance-issue}. 

\begin{wrapfigure}{r}{0.66\textwidth}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{balance_problem_c.pdf}
  \end{center}
  \caption{When $\mu_T \gg \mu_S$, the classifier $h_{w_c}(x) = \sigma \langle w, x\rangle$ is on the Pareto frontier of $\H_w$.}
  \label{fig:balance-issue2}
\end{wrapfigure}

The discussion above hints at one way forward: Looking at (b), $h_{w_b}$ is clearly preferred over $h_w$, as it is both more accurate and more balanced. This may suggest an alternative definition, that considers a classifier as ``kosher'' if it belongs to the \emph{Pareto frontier} of $\H$ with respect to balance and accuracy. That is, that it is the optimal classifier at a given allowed level of imbalance (see, e.g., \cite{1599245}). In our context however, more realistic scenarios reveal that this is not necessarily the end of the story. Consider the example in Figure \ref{fig:balance-issue2}, which is a variant of the examples we previously studied in Figure \ref{fig:balance-issue}. This time the classifier $h_{w_c}$ belongs to the Pareto frontier of $\H$,
because when $S$ is small compared to $T$, any improvement in balance will come at the cost of accuracy. This doesn't necessarily make $h_{w_c}$ desirable or fair: as we will discuss, the desired trade-off between balance and accuracy may be task-specific. 

Our definition of \gammafairness will address these issues. Intuitively, instead of objectively checking the imbalance of a certain predictor $h$ (and considering it okay if  it's, for  example, below a certain threshold), we will seek to  compare the imbalance of $h$ to the imbalance of predictors from a certain candidate class -- and deeming $h$  as fair if its current imbalance can't be improved by switching  to another predictor from this class (without \emph{significantly} hurting accuracy, as specified by an external parameter). As we will see, our notion generalizes both the usual notion of balance and the notion of Pareto efficiency described above. 



%Our definition of \fairness will aim  to address precisely  this issue. Intuitively, instead of objectively checking the imbalance of a certain predictor $h$ (and considering it okay if  it's, for  example, below a certain threshold), we will seek to  compare the imbalance of $h$ to the imbalance of predictors from a certain candidate class -- and deeming $h$  as fair if its current imbalance can't be improved by switching  to another predictor from this class (without significantly hurting accuracy).




\begin{exmp}
To build intuition regarding the notion of \emph{disqualification}, we return to the examples in Figure \ref{fig:balance-issue}. For simplicity, suppose $\ell_A = \ell_B = \ell$ are both the expected zero one loss and assume $\gamma = 1$. Recall that
in both (a) and (b), the classifier $h_w$ had an imbalance of 0.5. 
We will argue that out of the two candidates mentioned there, $h_{w_a}$ and $h_{w_b}$, only the second disqualifies $h_w$. Note that the losses are:

\begin{multicols}{2}
\noindent
\begin{gather*}
\textbf{(a)} \\ 
    \ell(h_w) \approx \mu_S \cdot 0.5 + \mu_T \cdot 0 = 0.25 \\
    \ell(h_{w_a}) \approx \mu_S \cdot 0.5 + \mu_T \cdot 0.5 = 0.5
\end{gather*}
\begin{gather*}
\textbf{(b)} \\ 
    \ell(h_w) \approx \mu_S \cdot 0.5 + \mu_T \cdot 0 = 0.25 \\
    \ell(h_{w_b}) \approx \mu_S \cdot 0.0 + \mu_T \cdot 0.0 = 0.0
\end{gather*}
\end{multicols}


So using $h' = h_{w_b}$, Equation (\ref{eqn:gamma-disq}) becomes

\begin{equation*}
    0.5 > f_1(\max \set{0, -0.25}) = f_1(0) = 0
\end{equation*}

which is true, so $h_{w_b}$ indeed disqualifies $h_w$. On the other hand, using $h' = h_{w_a}$, Equation (\ref{eqn:gamma-disq}) becomes

\begin{equation*}
    0.5 > f_1(\max \set{0, 0.25}) = f_1(0.25) = \frac{0.25}{\mu \cdot \beta} = \frac{0.25}{0.5 \cdot 0.5} = 1
\end{equation*}

which is not true. So  $h_{w_a}$, despite being significantly more balanced, 
does \emph{not}  disqualify $h_w$.  

\end{exmp}

Recall that part of our motivation of \fairness was the observation that balance itself cannot separate between intuitively different scenarios. However, there are still settings in which balance may be desirable.
As noted by \cite{hardt2016equality}, while intentionally worsening the performance on $T$ may seem non-sensical, this could be important from an incentives perspective: the willingness to use such a ``sanction''  places the burden of uncertainty in prediction on the decision-maker, thereby motivating them to invest towards more accurate predictions for the minority in the future. This highlights that balance could be desirable in the presence of a strategic (and discriminatory) decision-maker.  
On  the other hand,  there are other scenarios in which this behaviour is less appropriate, see e.g. \cite{chen2018my, blum2019advancing}. For example, in a medical scenario, the decision-maker is typically well-intentioned, but still cannot completely eliminate uncertainty regarding all groups (in that it is unrealistic to expect  perfect predictions for binary label $\Y$). In such a case it would arguably be unethical to  hurt the predictions for some individuals, in the name of balance. 
